One-Shot Coding and Applications

One-shot information theory addresses scenarios in source coding and channel coding where the signal blocklength is assumed to be 1. In this case, each source and channel can be used only once, and the sources and channels are arbitrary and not required to be memoryless or ergodic. We study the achievability part of one-shot information theory, i.e., we consider explicit coding schemes in the oneshot scenario. The objective is to derive one-shot achievability results that can imply existing (first-order and second-order) asymptotic results when applied to memoryless sources and channels, or applied to systems with memory that behave ergodically. Poisson functional representation was first proposed as a one-shot channel simulation technique by Li and El Gamal [118] for proving a strong functional representation lemma. It was later extended to the Poisson matching lemma by Li and Anantharam [117], which provided a unified one-shot coding scheme for a broad class of information-theoretic problems. The main contribution of this thesis is to extend the applicability of Poisson functional representation to various more complicated scenarios, where the original version cannot be applied directly and further extensions must be developed.

==> pages/abstract-zh.tex <==



\emph{單發信息论}探討的是信道编码与信源压缩在信號區塊長度1时的一般情境。在此情況下，每個信道與信源僅使用一次，且信道與信源都可以是任意的，並不被要求具備無記憶性或遍歷性。本論文的目標是構造出新的編碼方式，以推導出新的單發可達性結果。
當這些結果應用於無記憶的信道與信源或是有遍歷性的有記憶系統時，能夠推導出既有的一階與二階的漸近結果。\emph{泊松函數表示}作為一種單發信道模擬技術，最初由 Li 與 El Gamal 提出，用於證明強函數表示引理及其他結果。Li 與Anantharam 將其擴展為\emph{泊松配對引理}，並提供了一套能夠涵蓋廣泛的信息论問題的統一單發編碼方案。本論文的主要貢獻在於進一步擴展泊松函數表示與泊松配對引理的適用範圍，基於它們來設計新的工具和處理更為複雜的情境。下述分章節列舉本論文的幾個核心貢獻。

在第~\ref{chp:nnc}~章中，我們設計了一個針對任意無環噪聲網路中多個節點間資訊通 信與壓縮的統一框架。此框架可被視為 Lee 與 Chung 所研究之漸進隨機編碼 界限的單發對應版本，或者 Lim 等人所提出之噪聲網絡編碼的單發對應版本。 我們的編碼框架涵蓋極廣泛的網路信息论問題，不僅能復現多種既有的單發與漸近結果，亦提出了多種新的單發可達性結果。
在第~\ref{chp:hiding}~章中，我們基於泊松配對引理，探討了兩類與資訊安全相關的問題，其共同點和難點在於編碼器與解碼器需要在未知的信道狀態下編碼。我們對一般化的資訊隱藏問題與複合竊聽信道問題給出了新的單發可達性結果，並涵蓋了多種既有問題作為特例。
在第~\ref{chp:ppr}~章中，我們擴展了泊松函數表示，設計出一種用於壓縮任意差分隱私方法的新型結構，名為泊松隱私表示。泊松隱私表示是首個同時達成幾乎最佳的壓縮性能、精確無損的輸出分佈（從而保留原始隱私機制的統計性質，如無偏性與高斯性）、並確保差分隱私的構造。我們同時也於多種應用上展示了泊松隱私表示的實驗優勢。



